Formalising the Optimised Link State Routing Protocol

Routing protocol specifications are traditionally written in plain English. Often this yields ambiguities, inaccuracies or even contradictions. Formal methods techniques, such as process algebras, avoid these problems, thus leading to more precise and verifiable descriptions of protocols. In this paper we use the timed process algebra T-AWN for modelling the Optimised Link State Routing protocol (OLSR) version 2.

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{A. Fehnker and H. Garavel (Eds.):\\
Models for Formal Analysis of Real Systems (MARS 2020)\\
EPTCS 316, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.316.3}{10.4204/EPTCS.316.3}}
\pdfoutput=1
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{3}}{\finishreference{#1}{316}{\opa}{72}{120}{4}}{%
 this volume of #1\opa}}

